Interactive Interference Alignment

We study interference channels (IFC) where interaction among sources and destinations is enabled, e.g., both sources and destinations can talk to each other using full-duplex radios. The interaction can come in two ways: 1) {\em In-band interaction:} sources and destinations can transmit and listen in the same channel simultaneously, enabling interaction. 2) {\em out-of-band interaction:} destinations talk back to the sources on an out-of-band channel, possible from white-space channels. The flexibility afforded by interaction among sources and destinations allows for the derivation of interference alignment (IA) strategies that have desirable "engineering properties": insensitivity to the rationality or irrationality of channel parameters, small block lengths and finite SNR operations. We show that for several classes of interference channels the interactive interference alignment scheme can achieve the optimal degrees of freedom. In particular, we show the {\em first simple scheme} (having finite block length, for channels having no diversity) for $K=3,4$ that can achieve the optimal degrees of freedom of $\frac{K}{2}$ even after accounting for the cost of interaction. We also give simulation results on the finite SNR performance of interactive alignment under some settings. On the technical side, we show using a Gr\"{o}bner basis argument that in a general network potentially utilizing cooperation and feedback, the optimal degrees of freedom under linear schemes of a fixed block length is the same for channel coefficients with probability 1. Furthermore, a numerical method to estimate this value is also presented. These tools have potentially wider utility in studying other wireless networks as well.

==> converse.tex <==
Before we present the transmission scheme for interference channel with feedback, we first give the converse. More precisely, we will show that even with free feedback the sum degrees of freedom cannot exceed $\frac{K}{2}$. We borrow the proof from \cite{CJ2009}. For self-completeness, we give the converse proof in the following.

\begin{theorem}
	For a $K$-user interference channel where each transmitter can get free channel output feedback from all receivers, the sum degrees of freedom is upper bounded by $\frac{K}{2}$ for generic channel matrix $H$. 
\end{theorem}

\begin{IEEEproof}
We prove  $\sum_{i=1}^{K} d_i \le \frac{K}{2}$ by showing that for all $i \neq j$, 
\begin{align}
	d_i + d_j \le 1. \label{eqn:dof2}
\end{align}

By symmetry, we only need to consider the case $i=1$ and $j=2$.

The proof consists of two steps: in the first step, we construct a two user
MIMO interference channel, the sum degrees of freedom of which is no less than the original interference channel with feedback; in the second step, we bound the sum degrees of freedom of the two user MIMO interference channel by Fano's inequality.

\textbf{Step 1: } We assume all  transmitters except the first transmitter can fully cooperate with each other, and all receivers excepet the second receiver can fully cooperate with each other. Then, equivalently we get a two user MIMO interference channel, where both the second transmitter and the first receiver have $K-1$ antennas, while both the first transmitter and second receiver have a single antenna. Furthermore, we assume the messages $W_i$ are empty,  $ \forall i \ge 3$.

Since cooperation among transmitters and receivers cannot hurt the communication, an upper bound of the sum degrees of freedom $(d_1 + d_2)$ of the above two user MIMO interference channel is also a valid upper bound for the original $K$-user interference channel with feedback. 

\textbf{Step 2: } Next we use Fano's inequality to upper bound $d_1 + d_2$ by 1 in the two user MIMO interference channel, and thus show that feeedback and relay cannot increase the multiplexing gain of interference channel.

For the two user MIMO interference channel, we have the following input and output equaitons:
\begin{align}
\bar{Y}_1[t] &= \bar{H}_{11} X_1[t] + \bar{H}_{21}\bar{X}_2[t] + \bar{Z}_1[t] \\
Y_2[t] &= \bar{H}_{12} X_1[t] + \bar{H}_{22}\bar{X}_{2}[t] + Z_2 [t] ,
\end{align}
where
\begin{align}
X_1^t &= f_t (W_1, \bar{Y}_1^{t-1}, Y_2^{t-1}) \\
\bar{X}_2^t &= g_t (W_2, \bar{Y}_1^{t-1}, Y_2^{t-1} ),
\end{align}
for some encoding functions $f_t(\cdot)$ and $g_t(\cdot)$.

By Fano's inequality, we have
\begin{align}
 & N (R_1 + R_2 - \epsilon) \\
\le & I(Y_1^N ; W_1) + I(Y_2^N; W_2) \\
= & H(Y_2^N) - H(Y_2^N | W_2) + I(Y_1^N ; W_1)  \\
\le & H(Y_2^N) - H(Y_2^N | W_2) + I(Y_1^N, W_2; W_1 )  \\  % provide side information to receiver one
= & H(Y_2^N) - H(Y_2^N | W_2)  + I(Y_1^N; W_1 | W_2 ) \\  % since W1 and W_2 are independent
= & H(Y_2^N) - H(Y_2^N | W_2)  + H(Y_1^N | W_2) -   H(Y_1^N | W_1 , W_2 ) \\
\le &  H(Y_2^N) - H(Y_2^N | W_2)  + H(Y_1^N | W_2) \\
\le &  H(Y_2^N) - H(Y_2^N | W_2)  + H(Y_1^N, Y_2^N | W_2) \\
= & H(Y_2^N)  + H(Y_1^N | W_2 ,Y_2^N ).
\end{align}

The first term $H(Y_2^N)$ can be easily bounded by $N \log (SNR) + o(\log(SNR))$, and the second term can be upper bounded by
\begin{align}
& H(Y_1^N | W_2 ,Y_2^N ) \\
= & \sum_{t=1}^{N} H(Y_1[t] | W_2, Y_2^N, Y_1^{t-1}) \\
= & \sum_{t=1}^{N} H(Y_1[t] | W_2, Y_2^N, Y_1^{t-1}, X_2[t]) \\
= & \sum_{t=1}^{N} H(  \bar{H}_{11} X_1[t] + \bar{H}_{21}\bar{X}_2[t] + \bar{Z}_1[t]    | W_2, Y_2^N, Y_1^{t-1}, X_2[t]) \\
= &   \sum_{t=1}^{N} H(  \bar{H}_{11} X_1[t]  + \bar{Z}_1[t]   | W_2, Y_2^N, Y_1^{t-1}, X_2[t])            \\
\le &  \sum_{t=1}^{N} H(  \bar{H}_{11} X_1[t]  + \bar{Z}_1[t]   | Y_2[t], X_2[t])            \\
\le &  \sum_{t=1}^{N} H(  \bar{H}_{11} X_1[t]  + \bar{Z}_1[t]   |\bar{H}_{12} X_1[t] + Z_2 [t], X_2[t]) \\
\le &  \sum_{t=1}^{N} H(  \bar{H}_{11} X_1[t]  + \bar{Z}_1[t]   |\bar{H}_{12} X_1[t] + Z_2 [t]) \\
\le & N o(\log (SNR)).
\end{align}

Therefore,
\begin{align}
R_1 + R_2 - \epsilon \le \log (SNR) + o(\log (SNR)),
\end{align}
and thus $d_1 + d_2 \le 1$, i.e., equation \eqref{eqn:dof2} holds.

Take the sum of equation \eqref{eqn:dof2} over all $ 1 \le i\neq j \le K$, and we get
\begin{align}
	\sum_{i=1}^{K} d_i \le \frac{K}{2}.
\end{align}

\end{IEEEproof}


==> freefeedback.tex <==
Although feedback cannot improve the degrees of freedom beyond $\frac{K}{2}$, feedback can significantly simplify the transmission scheme to achieve the optimal $\frac{K}{2}$ degrees of freedom. In this section, we first present a simple optimal transmission scheme when immediate channel output feedback is free and available to all transmitters. Then we   discuss how to design interference alignment scheme when only limited feedback is available in next section.


We assume that every transmitter can get free feedback from all receivers. This assumption is valid when feedback channel is much better than the forward channel, so that immediate channel output feedback is available to all transmitters.

Consider the following simple three-phase transmission scheme which can achieve the optimal $\frac{K}{2}$ degrees of freedom:
\begin{itemize}
    \item Phase 1: All TXs send their independent symbols  simultaneously. Then RXs get $y = Hx + n$, where $n$ is additive noise.
    \item Phase 2: All TXs get immediate channel output feedback from all RXs, i.e., each TX get to know $y$.
    \item Phase 3: Now with free feedback $y$,  TXs can do coding over $y$ and send out $My$, where $M$ is a coding matrix. Then RXs will receive
    \begin{align}
      y' = HMy + \tilde{n} = HMHx + HMn + \tilde{n},
    \end{align}
    where $\tilde{n}$ is the new additive noise of this transmission.
\end{itemize}

For generic matrix $H$, we can assume $H$ is nonsingular. Therefore, if we choose the coding matrix $M$ to be
\begin{align}
  M \triangleq (H^{-1})^2,
\end{align}
then in Phase 3 RXs get $y' = x + \text{noise}$. So each RX gets the desired signal sent by the transmitter in the first phase without any interference. Since each transmitter is able to send a symbol to its corresponding receiver without interference using two transmissions, each TX-RX pair gets $\frac{1}{2}$ degrees of freedom, and thus in total this transmission scheme achieves the optimal $\frac{K}{2}$ degrees of freedom.



==> scheme_backup.tex <==

In practical communication system, free channel output feedback may not be available to all TXs and the main approach  to getting feedback is through the feedback channel from RXs to TXs,  either via simultaneous out of band transmission or via in band half-duplex transmission. Therefore, it is interesting to study how limited feedback can help design a simple and optimal transmission scheme.


%%%%%%%%%%%%%%%%% begin three phase figures
\begin{figure}[t]
\centering
\includegraphics[scale=0.7]{phase1.pdf}
\caption{Phase 1: All TXs send their independent symbols  simulatenously. And RXs get $y = H x + n$, where $n$ is the  additive noise of the channel.}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[scale=0.7]{phase2.pdf}
\caption{Phase 2: After receiving signals from TXs in phase1, all RXs scale $y$ and send back to TXs using the feedback channel. TXs  get $f = GD_1 y +  \tilde{n}$}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[scale=0.7]{phase3.pdf}
\caption{Phase 3: Now each TX has two sets of signals $x$ and $f$, and TXs can send out a linear combination of $x$ and $f$ to RXs via the forward channel.}
\end{figure}

%%%%%%%%%%%%%%%%% end of three phase figures


Consider the following simple three-phase transmission scheme for interference channel with limited feedback through feedback channel:

\begin{itemize}
  \item Phase 1: All TXs send their independent symbols  simulatenously. And RXs get $y = H x + n$, where $n$ is the  additive noise of the channel.
  \item Phase 2: After receiving signals from TXs in phase1, all RXs scale $y$ and send back to TXs using the feedback channel. TXs  get $f = GD_1 y +  \tilde{n}$.
  \item Phase 3: Now each TX has two sets of signals $x$ and $f$, and TXs can send out a linear combination of $x$ and $f$ to RXs via the forward channel. RXs get
  \begin{align}
    y' &= H(D_2 x + D_3 f) + \hat{n} \\
      & =  (HD_2 + HD_3 G D_1H) x + HD_3GD_1 n + HD_3 \tilde{n} + \hat{n}.
  \end{align}
\end{itemize}


Before discussing how to cancel all interferences at each receiver, we emphasize that on contrast to the case with free immediate channel output feedback, the coding matrices $D_1, D_2$ and $D_3$ have to be diagonal matrices. With free immediate channel output feedback, each transmitter knows each entry of $y$, i.e., the signals received at each receiver, so the transmitter can do coding over the entire vector $y$, and the coding matrix $M$ can be arbitrary. However, with limited feedback through the feedback channel, each transmitter  and each receiver only know what signals they sent out and received. Therefore, the coding matrices  $D_1, D_2$ and $D_3$ have to be diagonal, i.e., each node can only do coding over what signals it sent out and received.


To make RXs be able to decode desired signals, one possibility is that we choose diagonal matrices $D_1,D_2$ and $D_3$ such that
$(HD_2 + HD_3 G D_1H )$ is a diagonal matrix and every diagonal entry is nonzero, which makes each transmitter get the desired signal from $y'$ without interference. So the question is whether it always exists such $D_1,D_2$ and $D_3$.

Making all off diagonal entries to be zero gives us $K(K-1)$ polynomial equations, and each diagonal entry being nonzeros leads to $K$ inequalities, while in total we have $3K$ variables, which correspond to the diagonal coding matrices $D_1, D_2$ and $D_3$. One may conjecture that if the number of  variables is more than the number of equations, we may get a non trivial solution of  the polynomial equations, and make the $K$ inequalities hold.

Unfortunately, this conjecture is not true: in some cases, even if the number of variables is more than equations, due to the coupled constraints on the equations and inequalities, all off-diagonal entries of $(HD_2 + HD_3 G D_1H )$ being zero implies that at least one diagonal entry is zero. The simpliest counter example is
\begin{claim}
  For three-user interference channel with reciprocal feedback channel ($G = H^T$), for generic matrix $H$, there does not exist $D_1,D_2$ and $D_3$ such that $(HD_2 + HD_3 G D_1H )$ is a diagonal matrix and every diagonal entry is nonzero.
\end{claim}

% more explanation in next section on algebraic geometry

However, it is uncessary to make the transmission in Phase 3 completely interference-free. Since RXs have already got signals $y$ in the first phase, RXs can still cancel all interferences by taking a linear combiniation of $y$ and $y'$ if the interference terms in $y'$ are aligned with the interference terms in $y$.

More precisely, let $ B \triangleq HD_2 + HD_3 G D_1H $. Then for receiver $t_i$, in Phase 1 it receives
\begin{align}
  y_i = H_{ii} x_i + \sum_{j \neq i} H_{ij} x_j + \text{noise term},
\end{align}
and in Phase 3 it receives
\begin{align}
  y'_i = B_{ii} x_i + \sum_{j \neq i} B_{ij} x_j + \text{noise term}.
\end{align}

If for all $1 \le i \le K$, we have
\begin{align}
  \frac{B_{ij}}{H_{ij}} = \frac{B_{ij'}}{H_{ij'}} , \forall j,j'\neq i, \label{eqn:key1}
\end{align}
or equivalently
\begin{align}
  \frac{B_{ij}}{H_{ij}} = \lambda_i, \forall j \neq i,
\end{align}
for some constant $\lambda_i$,
then interference terms of $y$ and $y'$ for each receivers are aligned with each other. So receiver $t_i$ can compute $y_i - \lambda_i y'_i$ and get
\begin{align}
   (H_{ii} - \lambda_i* B_{ii})x_i + \text{noise term}.
\end{align}
Therefore, if $(H_{ii} - \lambda_i* B_{ii}) \neq 0$, or equivalently,
\begin{align}
  \frac{B_{ii}}{H_{ii}} \neq \frac{B_{ij}}{H_{ij}}, \forall j \neq i, \label{eqn:key2}
\end{align}
then RX $t_i$ gets the desired signal sent by TX $s_i$ without any interference.

Without introducing the auxiliary variables $\lambda_i$, aligning $K-1$ interference terms each receiver corresponds to $K-2$ equations, and thus in total we have $K(K-2)$ interference alignment equations. Preserving the desired signals after cancelling all interference terms leads to $K$ inequalities. Therefore, to make the three-phase communication scheme work and thus achieve the optimal $\frac{K}{2}$ degrees of freedom, we need to solve $K(K-2)$ equations with $3K$ variables and check that the solution satisfies  the $K$ inequalties.

\subsection{Three-User Interference Channel}

When $K=3$,  the number of variables is $3K = 9$, which is much more than the number of equations $K(K-2) = 3$, so it is not surprising that we can find  $D_1, D_2$ and $D_3$ to solve the above equations and inequalities.


First we state a lemma which will be used in the proof of Theorem \ref{thm:3user}.

\begin{lemma}\label{lem:dimension}
  Let $S_0 \subset \C^n$ be a linear subspace with dimension $d_0$. For any $m$ linear subspaces $S_1,S_2,\dots,S_m \subset S_0$ with dimensions $d_1,\dots,d_m$ respectively, if
  \begin{align}
    d_i < d_0, \forall 1 \le i \le m,
  \end{align}
  then $S_0 \backslash (\cup_{i=1}^m S_i)$ is a nonempty set.
\end{lemma}

\begin{IEEEproof}
  Let $e_1,\dots,e_{d_0} \in \C^n $ be a set of bases of $S_0$. Let $A \in \C^{d_0 \times d_0 m}$ such that every $d_0$ by $d_0$ submatrix of $A$ has full rank. It is easy to show the existence of $A$ with such property. Indeed, if every entry of $A$ is independently generated according to Gaussian distribution (or other continuous probability distributions), then with probability 1 every $d_0$ by $d_0$ submatrix of $A$ has full rank.

  Define $d_0 m$ vectors $b_1,b_2,\dots,b_{d_0 m}$ by setting
  \begin{align}
    b_i \triangleq \sum_{j=1}^{d_0} A_{ji} e_j,
  \end{align}
  for all $1 \le i \le d_0 m$.
  Since every $d_0$ by $d_0$ square submatrix of $A$ has full rank, every $d_0$ vectors of $b_1,b_2,\dots,b_{d_0 m}$ are linearly independent.

  Suppose $S_0 \backslash (\cup_{i=1}^m S_i)$ is a nonempty set, i.e., $S_0 = \cup_{i=1}^m S_i$. Then $b_1,b_2,\dots,b_{d_0 m} \in \cup_{i=1}^m S_i$. By pigeonhole principle, there exists $i^* \le d_0 m$ such that $S_{i^*}$ contains at least $d_0$ vectors of $b_1,b_2,\dots,b_{d_0 m}$. Since every  $d_0$ vectors of $b_1,b_2,\dots,b_{d_0 m}$ are linearly independent, the dimension of $S_{i^*}$ is no less than $d_0$, contradicting with the fact that $d_{i^*} < d_0$.

  Therefore, $S_0 \backslash (\cup_{i=1}^m S_i)$ is a nonempty set.

\end{IEEEproof}

\begin{theorem}\label{thm:3user}
  For three-user interference channel with reciprocal feedback channel ($G = H^T$), and for generic channel matrix $H$, there exists solutions to the interference alginment equations and inequalities.
\end{theorem}

\begin{IEEEproof}
The $K(K-2) = 3$ equations are
\begin{align}
  \frac{B_{12}}{H_{12}} &= \frac{B_{13}}{H_{13}}, \label{eqn:linear1} \\
  \frac{B_{21}}{H_{21}} &= \frac{B_{23}}{H_{23}}, \label{eqn:linear2} \\
  \frac{B_{31}}{H_{31}} &= \frac{B_{32}}{H_{32}}, \label{eqn:linear3}
\end{align}
and the $K = 3$ inequalities are
\begin{align}
  \frac{B_{11}}{H_{11}} &\neq \frac{B_{12}}{H_{12}}, \label{eqn:nonlinear1}\\
  \frac{B_{22}}{H_{22}} &\neq \frac{B_{23}}{H_{23}}, \label{eqn:nonlinear2}\\
  \frac{B_{33}}{H_{33}} &\neq \frac{B_{32}}{H_{32}},\label{eqn:nonlinear3}
\end{align}



  Since the number of variables is much more than the number of equations, we do not need to use all the variables. In fact, we can set $D_1$ to be a simple diagonal matrix
\begin{align}
  D_1 = \left(
  \begin{array}{ccc}
    1 & 0 & 0 \\
    0 & 0 & 0 \\
    0 & 0 & 0 \\
  \end{array}
\right).
\end{align}

Write $D_2$ and $D_3$ as
\begin{align}
  D_2 = \left(
  \begin{array}{ccc}
    D_{21} & 0 & 0 \\
    0 & D_{22} & 0 \\
    0 & 0 & D_{23} \\
  \end{array}
\right), \qquad
 D_3 = \left(
  \begin{array}{ccc}
    D_{31} & 0 & 0 \\
    0 & D_{32} & 0 \\
    0 & 0 & D_{33} \\
  \end{array}
\right).
\end{align}


Then equations \eqref{eqn:linear1}, \eqref{eqn:linear2} and \eqref{eqn:linear3} are homogeneous linear equations in terms of variables $D_{21}, D_{22}, D_{23}, D_{31}, D_{32}$ and $D_{33}$. Let $S$ denote the set of solutions to linear equations \eqref{eqn:linear1}, \eqref{eqn:linear2} and \eqref{eqn:linear3}. It is easy to check that the corresponding coefficient matrix has a rank of $3$. Therefore, $S$ is a linear subspace of dimension $6 - 3 = 3$.

Consider the following equations corresponding to the inequality constraints
\begin{align}
  \frac{B_{11}}{H_{11}} &= \frac{B_{12}}{H_{12}}, \label{eqn:linear4}\\
  \frac{B_{22}}{H_{22}} &= \frac{B_{23}}{H_{23}}, \label{eqn:linear5}\\
  \frac{B_{33}}{H_{33}} &=\frac{B_{32}}{H_{32}},\label{eqn:linear6}.
\end{align}

Let $S_1$ denote the set of solutions to \eqref{eqn:linear1}, \eqref{eqn:linear2}, \eqref{eqn:linear3} and \eqref{eqn:linear4}, let $S_2$ denote the set of solutions to \eqref{eqn:linear1}, \eqref{eqn:linear2}, \eqref{eqn:linear3} and \eqref{eqn:linear5},  and let $S_3$ denote the set of solutions to \eqref{eqn:linear1}, \eqref{eqn:linear2}, \eqref{eqn:linear3} and \eqref{eqn:linear6}. We can check that all the coefficient matrices of the linear equations
 have a rank of $4$, so all of $S_1, S_2$ and $S_3$ are linear subspaces of dimension $6 - 4 =2$.

 Now consider the set $S^* \triangleq S \backslash (S_1 \cup S_2 \cup S_3)$. Any element in $S^*$  satisfies both the equations \eqref{eqn:linear1}, \eqref{eqn:linear2}, \eqref{eqn:linear3}, and the inequality constraints \eqref{eqn:nonlinear1}, \eqref{eqn:nonlinear2}, \eqref{eqn:nonlinear3}.

 Since $S$ is linear subspace of dimension $3$, which is larger than the dimensions of $S_1, S_2$ and $S_3$, $S^*$ is a nonempty set by Lemma \ref{lem:dimension}. This completes the proof.

\end{IEEEproof}

% an alternative proof is that since the equations are linear, the solution has an analytical form, and thus we can plug the solution to the inequality and check whether inequality are satisfied.

The same result also holds when the feedback channel matrix is also a generic matrix  independent of $H$.








% next argue square root of K result

% simulations curves.

% H= D + uv^T result.




\subsection{Four-User Interference Channel}

For four-user interference channel, we have $K(K-2) = 8$ polynomial equation constraints and $K = 4$ inequality constraints with $3K = 12$ varaibles. We cannot use the same technique as in the case of three-user interference channel by setting $D_1$ or $D_3$ to be a deterministic constatn matrix and thus reducing the polynomial equations to linear equations. The reason is that if we do not use $D_1$ or $D_3$ as variables, the number of equations will be the same as the number of variables, and this will prevent us from finding a solution which also satisfies the inequality constraints.  Instead, we will use tools from algebraic geometry to check whether solution exists for the both equality and inequality constraints.

First, we show how to reduce the problem to checking the existence of solutions to polynomial equations.

Suppose there are $N$ polynomial equation constraints $f_i = 0$, $1 \le i \le N $, and $M$ polynomial inequality constraints $g_j \neq 0$, $1 \le j \le M$, over $S$ variables $\{d_1,d_2, \dots, d_S\}$. By introducing an auxiliary variable $t$, we define a polynomial function $\hat{g}$ as
\begin{align}
   \hat{g} \triangleq t\prod_{j=1}^M g_j - 1.
 \end{align}

 \begin{lemma}\label{lem:equivalence}
   There exists $(d_1,d_2, \dots, d_S)$ satisfying equality and inequality constraints
   \begin{align}
     f_i = 0 , \forall 1 \le i \le N \label{eqn:equalities}\\
     g_j \neq 0, \forall 1 \le j \le M, \label{eqn:inequalities}
   \end{align}
   if and only if there exists $(d_1,d_2, \dots, d_S, t)$ satisfying
    \begin{align}
     f_i = 0 , \forall 1 \le i \le N \label{eqn:newequalities}\\
     \hat{g} = 0. \label{eqn:newone}
   \end{align}
 \end{lemma}

\begin{IEEEproof}
  If $(d_1,d_2, \dots, d_S)$ is a solution to \eqref{eqn:equalities} and \eqref{eqn:inequalities}, then
  $(d_1,d_2, \dots, d_S, t)$ is a solution to \eqref{eqn:newequalities} and \eqref{eqn:newone}, where
  \begin{align}
    t \triangleq \frac{1}{\prod_{j=1}^M g_j}.
  \end{align}

  On the other hand, if $(d_1,d_2, \dots, d_S, t)$ is a solution to \eqref{eqn:newequalities} and \eqref{eqn:newone}, then $(d_1,d_2, \dots, d_S)$ satisfies both \eqref{eqn:equalities} and  \eqref{eqn:inequalities}.
\end{IEEEproof}
 % proof is straightforward


Therefore, due to Lemma \ref{lem:equivalence}, the problem of checking the existence of solutions to a system of polynomial equations and inequalities can be reduced to the problem of checking existence of solutions of a system of polynomial equations, which is well studied for algebraically closed field in algebraic geometry \cite{AGbook}. In the following we introduce some terminologies and main technical tools we will use in algebraic geometry. For more details on algebraic geometry, we refer the reader to the excellent textbook \cite{AGbook}.

We follow the standard notations in \cite{AGbook}.  Let $k$ denote a field, and use $k[x_1,x_2,\dots,x_n]$ denote the set of all polynomials in $x_1,x_2,\dots,x_n$ with coefficients in $k$.


\begin{definition}[Definition 1 on page 5 of \cite{AGbook}]
  Let $k$ be a field, and let $f_1,\dots,f_s$ be polynomials in $k[x_1,x_2,\dots,x_n]$. Then we call
  \begin{align}
    V(f_1,\dots,f_s) \triangleq \{ (a_1,\dots,a_n)\in k^n : f_i(a_1,\dots,a_n) = 0, \forall 1 \le i \le s\}
  \end{align}
  the \textbf{affine variety} defined by $f_1,\dots,f_s$.
\end{definition}


\begin{definition}[Definition 2 on page 30 of \cite{AGbook}]
  Let $f_1,\dots,f_s$ be polynomials in $k[x_1,x_2,\dots,x_n]$. Then we denote the ideal generated by $f_1,\dots,f_s$ as
  \begin{align}
    <f_1,\dots,f_s> \triangleq \{ \sum_{i=1}^s h_i f_i: h_1,\dots,h_s \in k[x_1,x_2,\dots,x_n] \}.
  \end{align}
\end{definition}

It is straightforward to see that $V(f_1,\dots,f_s) = V(<f_1,\dots,f_s>)$.

\begin{theorem}[ The Weak Nullstellensatz on page 170 of \cite{AGbook}]  \label{thm:nullstellensatz}
  Let $k$ be an algebraically closed field and let $I \subset k[x_1,x_2,\dots,x_n]$ be an ideal satisfying $V(I) = \emptyset$. Then $I = k[x_1,\dots,x_n]$.
\end{theorem}


\begin{corollary}\label{cor:1}
  Let $f_1,\dots,f_s$ be polynomials in $k[x_1,x_2,\dots,x_n]$, where $k$ is an algebraically closed field. Then $V(f_1,\dots,f_s) = \emptyset$ if and only if $1 \in <f_1,\dots,f_s>$.
\end{corollary}
\begin{IEEEproof}
  If $1 \in <f_1,\dots,f_s>$, then $<f_1,\dots,f_s> =  k[x_1,\dots,x_n]$, and thus $V(f_1,\dots,f_s) = V(<f_1,\dots,f_s>) = V(k[x_1,\dots,x_n]) = \emptyset$.

  On the other hand, if $V(f_1,\dots,f_s) = \emptyset$, eqvuivalently, $V(<f_1,\dots,f_s>) = \emptyset$, then by Theorem \ref{thm:nullstellensatz} we have
  \begin{align}
    <f_1,\dots,f_s> = k[x_1,\dots,x_n],
  \end{align}
  and thus $1 \in <f_1,\dots,f_s>$.

\end{IEEEproof}



Therefore, given polynomials $f_1,\dots,f_s \in k[x_1,\dots,x_n]$, where $k$ is an algebraically closed field, to check whether $V(f_1,\dots,f_s)$ is nonempty, i.e., whether there exists solution  to the system of polynomial equations
\begin{align}
  f_i = 0, \forall 1 \le i \le s,
\end{align}
 we only need to check whether $1 \in <f_1,\dots,f_s>$. This is the ideal membership problem, which is well studied in algebraic gemoetry. The basic tool we will use is \emph{Gr\"{o}bner basis} \cite{grobner}. Below we give a short introduction to \emph{Gr\"{o}bner basis} and show how to use \emph{Gr\"{o}bner basis} to solve the ideal membership problem.

 \begin{definition}[Definition 7 on page 59 of \cite{AGbook}]
   Let $f = \sum_{\alpha} a\_{alpha}x^{\alpha}$ be a nonzero polynomial in $k[x_1,\dots,x_n]$ and let $>$ be a monomial order. Then we define the \textbf{multidegree} of $f$ as
   \begin{align}
     multideg(f) \triangleq \max (\alpha: a_{\alpha} \neq 0 ),
   \end{align}
   where the maximum is taken with respect to the monomial order $>$.

   And we define the \textbf{leading term} of $f$ as
   \begin{align}
      LT(f) \triangleq a_{multideg(f)} x^{multideg(f)}.
   \end{align}

 \end{definition}

Given an ideal $I$, we use $LT(I)$ to denote the set of leading terms of elements of $I$, i.e.,
\begin{align}
  LT(I) \triangleq \{LT(f) |  f \in I  \}.
\end{align}


Due to Theorem \ref{thm:hilbert}, every ideal in $k[x_1,\dots,x_n]$ has a finite generating set.
\begin{theorem}[Hilbert Basis Theorem on page 76 of \cite{AGbook}] \label{thm:hilbert}
  Every ideal $I \subset k[x_1,\dots,x_n]$ has a finite generating set. That is, $I = <g_1,\dots,g_t>$ for some $g_1,\dots,g_t \in I$.
\end{theorem}


\begin{definition}[Definition 5 on page 77 of \cite{AGbook}]    % defintion of grobner basis, page 77
  Fix a monomial order. A finte subset $G = \{g_1,\dots,g_t\}$ of an ideal $I$ is said to be a \textbf{Gr\"{o}bner basis} if
  \begin{align}
    <LT(g_1), \dots, LT(g_t)> = <LT(I)>.
  \end{align}
\end{definition}

Equivalently, a set $\{g_1,\dots,g_t\} \subset I$  is a Gr\"{o}bner basis of $I$ if and only if the leading term of any element of $I$ is divisible by one of the $LT(g_i)$ \cite{AGbook}.

\begin{proposition}[Proposition 1 on page 82 of \cite{AGbook}]
  Let $G = \{g_1,\dots,g_t\}$ be a Gr\"{o}bner basis for an ideal $I \subset k[x_1,\dots,x_n]$ and let $f \in k[x_1,\dots,x_n]$. Then there is a unique $r \in k[x_1,\dots,x_n]$ with the following two properties:

  (i) No term of $r$ is divisible by any of $LT(g_1), \dots, LT(g_t)$.

  (ii) There is $g \in I$  such that $f = g + r$.

  In particular, $r$ is the remainder on division of $f$ by $G$ no matter how the elements of $G$ are listed when using the division algorithm.
\end{proposition}


An important property of  Gr\"{o}bner basis is that given a polynomial $f$, we check whether $f$ is in the corresponding ideal via division of $f$ by $G$. More precisely,

\begin{corollary}\label{cor:3}
  Let $G = \{g_1,\dots,g_t\}$ be a  Gr\"{o}bner basis for an ideal $I \subset k[x_1,\dots,x_n]$ and let $f \in k[x_1,\dots,x_n]$. Then $f \in I$ if and only if the remainder on division of $f$ by $G$ is zero.
\end{corollary}



\begin{corollary}\label{cor:2}
   Let $G = \{g_1,\dots,g_t\}$ be a Gr\"{o}bner basis for an ideal $I \subset k[x_1,\dots,x_n]$. Then $1 \in I$ if and only if
   \begin{align}
     g_i = \lambda,
   \end{align}
   for some $i \le t$ and nonzero $\lambda \in k$.
\end{corollary}

\begin{IEEEproof}
  We first prove the easier direction. If for some $i, g_i = \lambda \neq 0$, then $<g_i> =  k[x_1,\dots,x_n]$. So $I = k[x_1,\dots,x_n]$ and thus $1 \in I$.

  For the other direction, suppose that  $1 \in I$, but for each $i \le t$, the leading term of $g_i$ has a nonzero order, i.e., $g_i$ does not have the form $g_i = \lambda$ for some nonzero $\lambda \in k$. Then after we do division of $1$ by $G$, the remainder will be $1$, so the remainder is nonzero, and thus $1 \notin I$ by Corollary \ref{cor:3}, which leads to a contradiction. Therefore, for some $i$, $g_i$ can be written as  $g_i = \lambda$  for some nonzero $\lambda \in k$.
\end{IEEEproof}

Due to Corollary \ref{cor:1} and Corollary \ref{cor:2}, to check whether there exists solution to a system of polynomial equations over algebraically closed field, we only need to compute a Gr\"{o}bner basis of the corresponding ideal and check whether a nonzero scalar is in the Gr\"{o}bner basis.  We use standard  Buchberger's algorithm  \cite{Buchberger} to compute a Gr\"{o}bner basis.

Unfortunately, computing Gr\"{o}bner basis of a system of symbolic polynomails, where all coefficients in the polynomails are in symbolic form, is computationally expensive. Although, Buchberger's iterative algorithm can be proven to terminate in finite number of steps, it turns out to be computationally infeasible to run the algorithm for the symbolic polynomial equations in our problem.

However, it is much easier to compute a Gr\"{o}bner basis numerically. We do extensive numeric verfications: each time we generate random numeric channel matrices $H$ and $G$, and then apply Buchberger's algorithm to compute a  Gr\"{o}bner basis. In all numeric instances, the Gr\"{o}bner basis does not contain a nonzero scalar, which implies that solution to \eqref{eqn:key1} and \eqref{eqn:key2} exists.
%the main challenge is that after each step of  Buchberger's algorithm, the coefficient of each term in the new derived polynomail is in symbolic form and the length of

% add a theory explaining that numeric verification is sufficient.
% may be we need to rewrite the proof . First argue that why we do symbolic computation.
\begin{theorem}\label{thm:equivalsym_num}
  Let $f_1,\dots,f_s$ be polynomials in $k[x_1,x_2,\dots,x_n]$, where all coefficients of the polynomials are rational functions of variables $h_1,h_2,\dots,h_m$ in symbolic form. Let   $G = \{g_1,\dots,g_t\}$ be the symbolic Gr\"{o}bner basis for  $<f_1,\dots,f_s>$ obtained via Buchberger's algorithm. If we draw each $h_i$ according to a continuous probability distribution independently for all $ 1 \le i \le m$, and let  $G' = \{g'_1,\dots,g'_{t'}\}$ be the numeric Gr\"{o}bner basis for  $<f_1,\dots,f_s>$ obtained via Buchberger's algorithm, then with probability 1, $G'$ has the same structure as $G$.
\end{theorem}

\begin{IEEEproof}
Proof idea: Buchberger's algorithm has been proven to terminate in finite number of steps, and in each reduction step the structure of new derived polynomials only depends on whether the sum of some coefficients in the old polynomails is zero or not. For fixed finite number of rational functions $c_1,c_2,\dots,c_n$ of  $h_1,h_2,\dots,h_m$, if $h_1,h_2,\dots,h_m$ are drawn independently from a continuous probability distribution and let $c'_i$ be the corresponding numeric value of $c_i$, then with probability 1, $c_i$ is zero polynomial if and only if $c'_i = 0$ for all $1 \le i \le n$. Therefore, with probability 1, $G$ and $G'$ have the same structures.
\end{IEEEproof}



Due to Theorem \ref{thm:equivalsym_num}, although we cannot compute a symbolic Gr\"{o}bner basis explicitly, from numeric verifications we believe  the following claims hold.

\begin{claim}
  For four-user interference channel with reciprocal feedback channel ($G = H^T$), for generic matrix $H$, there exists $D_1,D_2$ and $D_3$ such that each row of $(HD_2 + HD_3 G D_1H )$ is proportional to the corresponding row of $H$ except the diagonal entries.
\end{claim}

\begin{claim}
  For four-user interference channel with out of band feedback channel, for generic matrices $H$ and $G$, there exists $D_1,D_2$ and $D_3$ such that each row of $(HD_2 + HD_3 G D_1H )$ is proportional to the corresponding row of $H$ except the diagonal entries.
\end{claim}


\subsection{Beyond Four-User Interference Channel with Limited Feedback}

Recall that the number of variables $N_v$ is $3K$, the number of equations $N_e$ is $K(K-2)$ and the number of inequalities $N_{ie}$ is $K$. $N_e$ grows faster than $N_v$ as $K$ increases, and when $K \ge 5$, $N_v \le N_e$. We expect that when the number of variables is not more than the number of inequations, a valid solution may not exist. Indeed, we confirm this conjecture for $K = 5$ and $6$ via computing Gr\"{o}bner basis for random numeric $H$ and $G$ and finding that $1$ is in the Gr\"{o}bner basis in all instances.


\begin{claim}
  For $K$-user interference channel with reciprocal feedback channel ($G = H^T$) where $K=5$ or $6$, for generic matrix $H$, there does not exist $D_1,D_2$ and $D_3$ such that each row of $(HD_2 + HD_3 G D_1H )$ is proportional to the corresponding row of $H$ except the diagonal entries.
\end{claim}


\begin{claim}
  For $K$-user interference channel with out of band feedback feedback channel where $K=5$ or $6$, for generic matrices $H$ and $G$, there does not exist $D_1,D_2$ and $D_3$ such that each row of $(HD_2 + HD_3 G D_1H )$ is proportional to the corresponding row of $H$ except the diagonal entries.
\end{claim}


Since one reverse transmission from RXs to TXs is not enough, in Phase 2 we can let receivers make more than one reverse transmissions to TXs. In one extreme case, if each receiver sends what it receives in Phase 1 to all transmitters sequentially, where in total we use $K$\footnote{In fact, $K - 1$ is also sufficient.} reverse transmissions, then it will be reduced to the case of interference channel with full feedback.

It turns out that when $K =5$ or $K = 6$, two reverse transmissions in Phase 2 is sufficient to do interference alignment while still preserving the desired signals. A natural three-phase scheme is as follows:
\begin{itemize}
  \item Phase 1: All TXs send their independent symbols  simulatenously. And RXs get $y = H x + n$, where $n$ is the  additive noise of the channel.
  \item Phase 2-1: After receiving signals from TXs in phase1, all RXs scale $y$ and send back to TXs using the feedback channel. TXs  get $f^1 = GD_1 y +  \text{noise}$.
  \item Phase 2-2: All RXs scale $y$ using a different coding matrix and send back to  TXs. TXs get $f^2 = GD_2 y +  \text{noise}$.
  \item Phase 3: Now each TX has three sets of signals $x, f^1$ and $f^2$, and TXs can send out a linear combination of $x, f^1$ and $f^2$ to RXs via the forward channel. RXs get
  \begin{align}
    y' &= H(D_3 x + D_4 f^1 + D_5 f^2) + \text{noise} \\
      & =  (HD_3 + HD_4 G D_1H + HD_5 G D_2H ) x + \text{noise}.
  \end{align}
\end{itemize}


With two reverse transmissions, the number of variables is increased to $5K$ from $3K$, and is more than $N_e = K(K-2)$ for $K = 5,6$. Extensive numeric simulations show that for generic matrix $H$ and $G$, there exists diagonal coding matrices $\{D_i\}_{1\le i \le 5}$ to align interferences while still preserving desired signals.


\begin{claim}
  For $K$-user interference channel with  reciprocal feedback channel ($G = H ^T$) where $K=5$ or $6$, for generic matrices $H$, there  exists $D_1,D_2, D_3, D_4$ and $D_5$ such that each row of $(HD_3 + HD_4 G D_1H + HD_5 G D_2H )$ is proportional to the corresponding row of $H$ except the diagonal entries.
\end{claim}


\begin{claim}
  For $K$-user interference channel with  out of band feedback channel where $K=5$ or $6$, for generic matrices $H$ and $G$, there  exists $D_1,D_2, D_3, D_4$ and $D_5$ such that each row of $(HD_3 + HD_4 G D_1H + HD_5 G D_2H )$ is proportional to the corresponding row of $H$ except the diagonal entries.
\end{claim}



\subsection{Numeric Finite SNR Performance Evaluation}

In this section, we present simulation results on the finite SNR performance of our three-phase interactive interference alignment scheme with out of band feedback transmissions  over i.i.d. Rayleigh-fading channels for $K = 3$ and $4$. We assume both transmitters and receivers have the same power constraint. We formulate the problem as a nonconvex optimization problem, and use generic local algorithm to maximize the sum rates among all possible interfernce alignment solutions while satisfying power constraints. For each SNR, we simulate over 50 channel realizations and compute the average of maximum sum rates. We compare the maximum rates achieved via interactive interference alignment with the standard time sharing scheme.




\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{K_3.pdf}
\caption{Numeric Finite SNR Performance Simulations for Three-User Interference Channel with Out of Band Feedback Channel}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{K_4.pdf}
\caption{Numeric Finite SNR Performance Simulations for Four-User Interference Channel with Out of Band Feedback Channel}
\end{figure}

For $K=3$ and $K = 4$, our interactive interference alignment scheme can achieve the optimal $\frac{K}{2}$ degrees of freedom, while time sharing scheme only gets $1$ degree of freedom. Therefore, at high SNR, we expect our scheme has  fifty percent improvement for $K = 3$ and $100\%$ percent improvement for $K=4$ over time sharing scheme, and this matches our simulation results.
% From the simulation curves, we can we can see that among all SNR from $0dB$ to $70dB$  
